Learning Constraints from Demonstrations

We extend the learning from demonstration paradigm by providing a method for learning unknown constraints shared across tasks, using demonstrations of the tasks, their cost functions, and knowledge of the system dynamics and control constraints. Given safe demonstrations, our method uses hit-and-run sampling to obtain lower cost, and thus unsafe, trajectories. Both safe and unsafe trajectories are used to obtain a consistent representation of the unsafe set via solving an integer program. Our method generalizes across system dynamics and learns a guaranteed subset of the constraint. We also provide theoretical analysis on what subset of the constraint can be learnable from safe demonstrations. We demonstrate our method on linear and nonlinear system dynamics, show that it can be modified to work with suboptimal demonstrations, and that it can also be used to learn constraints in a feature space.

==> method_back.tex <==
\section{Method}\label{sec:method}

The key to our method lies in finding lower cost trajectories that do not violate the known constraints, given a demonstration satisfying all constraints with optimal or boundedly-suboptimal cost. Such trajectories must then violate the unknown constraint. Our goal is to extract information about the location of unsafe states from these trajectories. We provide a brief outline of our method as follows:

\begin{enumerate}
	\item Form the set of trajectories that are of lower cost and are consistent with the known constraints
	\item Sample unsafe trajectories from this set via 1) a hit-and-run method and via 2) sampling local perturbations
	\item Solve an optimization problem and/or use side information to find a constraint that is consistent with the demonstrations and the unsafe trajectories.
\end{enumerate}

\subsection{Intersections with known constraints}

Some types of known constraints that we explicitly consider in this paper are the underlying dynamics of the system and the control limits. In particular, we detail our method for recovering constraints from trajectories generated by both linear and nonlinear dynamical systems subject to control constraints.

Let's consider a forward problem of the form described in Section \ref{sec:problem_statement}. We define the set of unsafe state-control trajectories induced by an optimal, safe demonstration $\traj_{xu}^*$, $\unsafetrajset$, as the set of state-control trajectories of lower cost that obey the known constraints:
\begin{equation}
	\unsafetrajset \doteq \{ \xi \ |\ c(\trajx, \traju) < c(\trajx^*, \traju^*), \xi \in \safeset^{\traj, k} \}
\end{equation}

In this paper, we work in particular with sets of known constraints that are due to the system dynamics and control constraints; so $\safeset^{\traj, k} = \dynfeasibleset \cap \controlfeasibleset$, where $\dynfeasibleset$ denotes the set of dynamically feasible state-control trajectories and $\controlfeasibleset$ denotes the set of state-control trajectories that use controls drawn from $\controlset$ at each time-step. We will develop the method for discrete time trajectories, but analogous definitions hold for the continuous time case.

For discrete time trajectories of length $T$, an explicit expression for $\controlfeasibleset$ is:
\begin{equation}
	\controlfeasibleset \doteq \{ \xi_{xu} \ |\ \control_1 \in \controlset, \ldots, \control_{T-1} \in \controlset\}
\end{equation}

Explicit expressions of $\dynfeasibleset$ for different classes of dynamics will be discussed in the following sections, as well as different methods for sampling them. We organize the methods in Table \ref{tbl:sampling}. Some more concrete examples follow, and Figures \ref{fig:dyn_umax} and \ref{fig:cost_ellipsoid} show simple examples of $\dynfeasibleset$ and $\controlfeasibleset$, and $c(\xi) < c(\xi^*)$, respectively. 

\begin{center}
\begin{table}
\begin{center}
\begin{tabular}{ | c | c | c | c | } 
\hline
Dynamics & Cost function & Control constraints & Sampling method \\ \hline
Linear & Quadratic & Convex & Ellipsoid hit and run (Section \ref{sec:elllipsoidsampling}) \\ \hline
Linear & Convex & Convex & Convex hit and run (Section \ref{sec:convexcost}) \\ \hline
\multicolumn{3}{| c |}{Else} & Non-convex hit and run (Section \ref{sec:nonconvexintersection}) \\ 
\hline
\end{tabular}
\end{center}
\caption{Sampling methods for different cost function / dynamics / control constraint combinations.}
\label{tbl:sampling}
\end{table}
\end{center}

\begin{figure}
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{dyn_umax_intersection}
  \caption{$\dynfeasibleset$ is shown for when $\state_{t+1} = 5\state_t + \control_t$, where $\state_t, \control_t \in \mathbb{R}$, for all $t$. $\controlfeasibleset$ is shown for when $\control_t \in [-1, 1]$, for all $t$.}
  \label{fig:dyn_umax}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{dyn_umax_intersection_nonlinear}
  \caption{$\dynfeasibleset$ is shown for when $\state_{t+1} = 10 \sin(\state_t) + \control_t$, where $\state_t, \control_t \in \mathbb{R}$, for all $t$. $\controlfeasibleset$ is shown for when $\control_t \in [-1, 1]$, for all $t$.}
  \label{fig:dyn_umax_nonlinear}
\end{minipage}%
\end{figure}

%\begin{wrapfigure}{r}{0.4\textwidth}
%  \centering
%  \includegraphics[width=\linewidth]{cost_ellipsoid_1d}
%  \caption{The unsafe set induced by demonstration $\traj^*$, $\unsafetrajset$, is plotted in red. No control constraints; dynamics: $\state_{t+1} = \state_t + \control_t$; cost function: $c(\state_1, \state_2, \state_3) = \sum_{t=1}^2 \vert \state_{t+1} - \state_t \vert$; all trajectories constrained so $\state_1 = 2$ and $\state_3 = 1$.}
%  \label{fig:cost_ellipsoid}
%\end{wrapfigure}

%Let's consider a forward problem with a quadratic objective function $\sum_{t=1}^{T-1} \Vert u_t \Vert_2^2$ that minimizes control effort, with linear dynamics $\state_{t+1} = A \state_t + B \control_t$, with control restricted to lie in $\controlset$, and with $\state_0$ and $\state_T$ being restricted to be the start and goal states, $\state_s$ and $\state_f$.

\subsubsection{Linear dynamics, convex control constraints, convex cost function}

In case the system has linear dynamics, the set of dynamically feasible state-control trajectories can be described as an eigenspace of a singular ``dynamics consistency" matrix, $\dynproject_1$, which converts any arbitrary state-control trajectory to one that satisfies the dynamics, one time-step at a time. Precisely, when the dynamics are in the form $\state_{t+1} = A\state_t + B\control_t$, we can write a matrix $\dynproject_1$ that fixes the controls and the initial state and changes the second state in the infeasible trajectory to the state that the system should be at if it is at state $\state_1$ and $\control_1$ is applied:

\begin{equation}
	\underbrace{\begin{bmatrix}
		\state_1 \\ \control_1 \\ \state_2 \\ \control_2 \\ \tilde{\state}_3 \\ \vdots
	\end{bmatrix}}_{\hat\xi_{xu}} = \underbrace{\begin{bmatrix}
		I & 0 & 0 & 0 & 0 & \cdots \\
		0 & I & 0 & 0 & 0 & \cdots \\
		A & B & 0 & 0 & 0 & \cdots \\
		0 & 0 & 0 & I & 0 & \cdots \\
		0 & 0 & A & B & 0 & \cdots \\
		\vdots & \vdots & \vdots & \vdots & \vdots & \ddots \\
	\end{bmatrix}}_{\dynproject_1} 
	\underbrace{\begin{bmatrix}
		\state_1 \\ \control_1 \\ \tilde{\state}_2 \\ \control_2 \\ \tilde{\state}_3 \\ \vdots
	\end{bmatrix}}_{\xi_{xu}}
\end{equation}

Here, we use a $\tilde{x}$ to denote a state that is dynamically infeasible with respect to the earlier state-control trajectory. If we multiply $\hat\xi_{xu}$ again by $\dynproject_1$, $\state_3$ will be converted to the dynamically feasible state. Following this logic, applying $\dynproject_1$ to the original $T$-time-step infeasible trajectory $T-1$ times results in a dynamically feasible trajectory:

\begin{equation}
	\xi_{xu}^\text{feas} = \dynproject_1^{T-1} \xi_{xu}
\end{equation}

We also note that the set of all dynamically feasible state-control trajectories is 
\begin{equation}
\dynfeasibleset \doteq \{ \xi_{xu} \ |\ \dynproject_1 \xi_{xu} = \xi_{xu} \}	
\end{equation}

\noindent which is the span of the eigenvectors of $\dynproject_1$ associated with eigenvalue $1$.

Then the set of unsafe trajectories can be defined as

\begin{equation}
	\unsafetrajset_{\text{linear}} \doteq \{ \xi_{xu} \ |\ c(\xi_{xu}) < c(\xi_{xu}^*), \xi_{xu} \in \dynfeasibleset, \xi_{xu} \in \controlfeasibleset \}
\end{equation}

Since $c(\xi) < c(\xi^*)$ is convex as it is a sub-level set of a convex function, $\dynfeasibleset$ is convex since it is a linear subspace, and $\controlfeasibleset$ is an intersection of convex sets since $\controlset$ is convex, the intersection of the three is also convex.

In particular, in the case where the objective function is quadratic, the sub-level sets become ellipsoids of the form $\xi_{xu}^\top V \xi_{xu} \le c^*$, where $V$ is a square matrix holding the ellipsoid parameters, with dimensions compatible with the state-control trajectory. In this case, the intersection of the sub-level set and the linear dynamics simplifies nicely to:

\begin{equation}\label{eq:ellipsoidset}
	\unsafetrajset_{\text{ellipsoid}} \doteq \{\xi_{xu} \ |\ \xi_{xu}^\top \dynproject_1^{{T-1}^\top} V \dynproject_1^{T-1} \xi_{xu} \le c(\xi_{xu}^*), \xi_{xu} \in \controlfeasibleset \}
\end{equation}

\subsubsection{Nonlinear dynamics or non-convex constraints}

When the system is instead described by general nonlinear dynamics of the form $\state_{t+1} = f(\state_t, \control_t)$, the intersection is in general no longer convex, since $\dynfeasibleset_\text{nonlinear}$ can now be an arbitrary non-convex manifold (see Figure \ref{fig:dyn_umax_nonlinear}). A similar non-convex intersection can result if the feasible control set $\controlset$ is non-convex, the cost function $c(\cdot)$ is non-convex, or both. The intersection in this non-convex case is

\begin{equation}
	\unsafetrajset_{\text{nonlinear}} \doteq \{ \xi_{xu} \ |\ c(\xi_{xu}) < c(\xi_{xu}^*), \xi_{xu} \in \dynfeasibleset_\text{nonlinear}, \xi_{xu} \in \controlfeasibleset \}
\end{equation}

\noindent where $\dynfeasibleset_\text{nonlinear}$ is described by

\begin{equation}
\dynfeasibleset_\text{nonlinear} \doteq \{ \xi_{xu} \ |\ \state_{t+1} = f(\state_t, \control_t), \control_t \in \controlset,  \forall t\}	
\end{equation}

We discuss techniques to sample trajectories from $\unsafetrajset_{\text{linear}}, \unsafetrajset_{\text{ellipsoid}}$, and $\unsafetrajset_{\text{nonlinear}}$ in Section \ref{sec:sampling}.

\subsection{Sampling the intersections}\label{sec:sampling}

Hit-and-run sampling \cite{hit_and_run} is a method for sampling sets that guarantees convergence to a uniform distribution over the set in the limit; the algorithm is shown in Algorithm \ref{alg:hnr}. We describe how the algorithm simplifies for the three cases mentioned in the previous section.

\begin{algorithm}\label{alg:hnr}
\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Output{$\textsf{out} \doteq \{\traj_1, \ldots, \traj_{\numunsafe}\}$}
\Input{$\unsafetrajset, \traj^*, \numunsafe$}
% \tcc{Get sub-level set}
% $\unsafetrajset \leftarrow \{ \traj | \ c(\traj) < \traj^*\}$\;
 $\traj \leftarrow \traj^*$\;
 $\textsf{out} \leftarrow \{ \}$\;
 \tcc{Sample sub-level set}
 \For{i = 1:$\numunsafe$}{
  \tcc{Sample random vector}
  $r \leftarrow $ rand\_dir\;
  \tcc{Compute line containing random direction and intersection with sub-level set}
  $\mathcal{L} \leftarrow \unsafetrajset \cap \{\xi' \in \trajset \ |\ \xi + \beta r\}$\;
  $L_-, L_+ \leftarrow \textsf{endpoints}(\mathcal{L})$\;
  $\traj \sim \textsf{Uniform}(L_-, L_+)$\;
  $\textsf{out} \leftarrow \textsf{out} \cup \traj$\;
 }
 \caption{Sampling infeasible trajectories via hit-and-run}
\end{algorithm}

\subsubsection{Linear dynamics and quadratic cost function}\label{sec:elllipsoidsampling}

We would like to sample from the set in Equation \ref{eq:ellipsoidset}. For now, let's ignore the control constraints and develop a method for sampling from $\{\xi_{xu} \ |\ \xi_{xu}^\top \dynproject_1^{{T-1}^\top} V \dynproject_1^{T-1} \xi_{xu} \le c(\xi_{xu}^*) \}$. 

We will use the hit-and-run algorithm described in Algorithm \ref{alg:hnr} to sample the set. Roughly, hit-and-run works as follows: after initializing the algorithm with a point within the set, repeatedly choose a direction in the ambient space uniformly at random, move a random amount in that direction such that the new point remains within the set, and set the new initial point to the point just sampled. 

When hit-and-run is used to sample from an ellipsoid, line 5 in Algorithm \ref{alg:hnr} simplifies, as we can very efficiently solve the quadratic equation 

\begin{equation}\label{eqn:hnr_ellipsoid}
	(\xi_{xu} + \beta r)^\top \dynproject_1^{{T-1}^\top} V \dynproject_1^{T-1} (\xi_{xu}  + \beta r) - c(\xi_{xu}^*) = 0
\end{equation}

\noindent for $\beta$, where $r$ is a random direction in the state-control trajectory space and $\beta \in \mathbb{R}$ is a scalar, to find the endpoints of the line segment to be sampled, $\mathcal{L}$.

We deal with control constraints separately because the intersection of $\controlfeasibleset$ and the ellipsoid, while convex, is in general no longer an ellipsoid. To deal with the control constraints, it is possible to project each sampled state-control trajectory onto the set of feasible controls. However, since it is possible for the sample to be projected outside of the intersection of the sub-level set and the dynamics eigenspace, we find in our experience that it is faster computationally to reject the samples that violate control constraints and continue sampling.

Additionally, to ensure that the start and goal constraints are obeyed for all sampled trajectories, we add an additional term to the cost function that adds a high penalty for the distance between the first state and start and the last state and goal: $\tilde{c}(\cdot) \doteq c(\cdot) + \alpha_c(\Vert \state_s - \state_1 \Vert_2^2 + \Vert \state_g - \state_T\Vert_2^2)$, where $\alpha_c$ is a large scalar.

\subsubsection{Linear dynamics and general convex cost function}\label{sec:convexcost}

For the case of a general convex cost function, the same procedure holds from the previous section, except we cannot directly solve the quadratic equation. To find $\mathcal{L}$, we need to solve $c(\xi_{xu} + \beta r) = 0$ to find $\mathcal{L}$'s endpoints. This can be done via a root finding algorithm or by doing a simple line search.

\subsubsection{Non-convex intersection}\label{sec:nonconvexintersection}

In the case of a non-convex intersection, $\mathcal{L}$ can now in general be a union of disjoint line segments, so the methods from before will not work well in general. In this scenario, we perform a ``backtracking" line search by setting $\beta$ to lie in some initial range: $\beta \in [\underbar{$\beta$}, \overline{\beta}]$; sampling $\beta_s$ within this range and then evaluating the cost function to see whether or not $\xi_{xu} + \beta_s r$ lies within the intersection. If it does, the sample is kept and hit-and-run proceeds like normal; if not, then the range of possible $\beta$ values is restricted to $[\beta_s, \overline\beta]$ if $\beta_s$ is negative, and $[\underbar{$\beta$}, \beta_s]$ else. Then, a new $\beta$ is re-sampled, and the process repeats, until either the interval shrinks below a sufficiently small size or a feasible sample is found.

\subsubsection{Sampling continuous time trajectories}

We make a brief note about sampling continuous time state-control trajectories. While hit-and-run can work for sampling in high dimensional spaces, sampling functions requires sampling in an infinite dimensional space, which is computationally infeasible. One can sidestep this by sampling piecewise constant control sequences (i.e. sampling control actions and durations for which to apply them $\control = \control_c, \forall t \in [t_1, t_2]$); then, applying these control sequences to a known initial condition can recover a continuous time state trajectory and a piecewise constant continuous control trajectory.

\subsection{Version space analysis}

As will be discussed further in Section $\ref{sec:analysis}$, learnability determines how much of a constraint can be recovered from safe demonstrations. How close our algorithm comes to the theoretical limit of learnability down to the ``quality" of the information encoded in the sampled trajectories, which we will now discuss.

Consider a length-$T$ discrete-time trajectory which is determined to be unsafe, $\xi$, which starts at $\state_s$ and ends at $\state_g$, both of which are in the safe set. All this means is that there exists at least one state in the trajectory which is unsafe: this information tells us nothing directly about which state was unsafe. This is inherent to the problem of determining information about an unsafe set when only given demonstrations in the safe set - the safe trajectories themselves provide no direct information about the location of the unsafe state(s). More concretely, in $\xi$, there exist at least $T-2$ states that could be unsafe: $\occ(\state_2) = 1 \vee \ldots \vee \occ(\state_{T-1}) = 1$.

The weakness of this information can be made concrete using a version space analysis, which is defined next: 

\begin{definition}[Version space]
	In a machine learning context, the version space is the set of consistent hypotheses (logical statements), given a set of constraints in the form of examples or training data \cite{versionspace}. In our setting, the space of hypotheses is the space of possible unsafe sets, and the constraints are the safe and unsafe trajectories.
\end{definition}

From the version space perspective, we can see how this information is relatively weak. The above constraint only disallows unsafe sets that mark all of the occupancies in that trajectory as safe: $\occ(\state_2) = 1 \wedge \ldots \wedge \occ(\state_{T-1}) = 1$. If the constraint is gridded into $G$ cells, this information invalidates $2^{G-T+2}$ possible unsafe sets in the binary constraint case. While this may seem like we removed many possible constraints, we could do exponentially better if we reduced the number of cells that the unsafeness is ``or"-ed over - the difference is especially pronounced if $T$ is large. In our experience, this level of information is often insufficient for quality recovery of the constraint.

\subsection{Reducing the learnability gap by exploiting cost function structure}

To improve upon the na\"ive approach of sampling only full-length trajectories, we will sample sub-segments (or sub-trajectories) of the larger demonstrations. This is motivated by the following example - if for a trajectory $\xi$ of length $T$, we fix all but one of the points on $\xi$ when sampling unsafe trajectories. Since only one state is different from the known safe demonstration, the unsafeness of the trajectory can be uniquely localized to whatever new point was sampled: then, this trajectory will reduce the version space by a factor of $2$, invalidating $2^{G-1}$ unsafe sets. 

Following this, for the case of the length-$T$ trajectory $\xi$, we can sample unique sub-trajectories of length $3, \ldots, T$, holding different sub-segments of the original demonstration fixed.

One can sample these sub-trajectories in the original high-dimensional state-control trajectory space without restriction, but to speed up the sampling, sub-trajectories can be sampled directly in the lower dimensional sub-trajectory state-control space if the cost function $c(\cdot)$ that is being optimized is strictly monotone \cite{monotonicity}:

\begin{definition}[Strict monotonicity]
	For any costs $c_1, c_2 \in \mathbb{R}$, control $\control \in \controlset$, and next state $\state \in \statespace$, the following holds:
	\begin{equation}
		c_1 < c_2 \Rightarrow h(c_1, \state, \control) < h(c_2, \state, \control), \forall \state, \control
	\end{equation}
	\noindent where $h(c, \state, \control)$ represents the cost of starting with initial cost $c$ at state $\state$ and taking control $\control$.
\end{definition}

Strictly monotone cost functions include separable cost functions with additive or multiplicative stage costs, which are common assumptions on the cost function in many motion planning and optimal control algorithms. If the cost function is strictly monotone, it makes sense to sample lower cost trajectories from sub-segments of the optimal path; otherwise it could be possible that even if a new sub-segment with lower cost than the original sub-segment were to be sampled, the full trajectory with the sub-segment replaced could have a higher cost than the demonstration. 

%If strict monotonicity holds, in our example $\xi$, we can sample trajectories of length $3, \ldots, T$. Unsafe trajectories coming from this procedure can provide exponentially more information: for example, in the case where we sample trajectories of length $3$, while holding the first and last state to be fixed on the demonstration, any trajectories that lie in the intersection will tell us that the middle state is uniquely unsafe - reducing the version space by a factor of $2^{G-1}$.

\subsection{Integer program formulation}\label{sec:integer_program}

The process described in the previous sections is summarized in Algorithm $\ref{alg:complete}$ and can be repeated for multiple given safe demonstrations.

Ultimately, this process will result in $\numsafe$ safe demonstrations and $\numunsafe$ unsafe sampled trajectories. Then, following the gridding procedure described in Section \ref{sec:inverse_problem} and interpreting the trajectories as constraints in an optimization problem results in the binary integer feasibility problem described in Equation \ref{eq:feasibility_program}.

%The $\numsafe$ given safe trajectories and the $\numunsafe$ sampled unsafe trajectories can together be thought of as a set of constraints on the possible locations of unsafe states. To recover an unsafe set that is consistent  with these constraints, we first discretize the constraint space into a finite set of $G$ discrete cells $\gridspace \doteq \{\grid_1, \ldots, \grid_G\}$ and define an occupancy function, $\occ(\cdot)$, which maps each cell to its safeness: $\occ(\cdot) : \gridspace \rightarrow \{0, 1\}$, where $\occ(\grid_i) = 1$ if $\grid_i$ is determined to be unsafe, and $0$ else. The gridded analogue of the continuous space trajectories is generated by concatenating the set of grid cells $\grid_i$ that the trajectory $\state_1, \ldots, \state_T$ lies in, which is graphically shown in Figure \ref{fig:discretization}. 

%Interpreting these safe and unsafe trajectories as constraints in an optimization problem, we can pose a binary integer feasibility problem that recovers an unsafe set consistent with the trajectories:
%
%\begin{equation}\label{eq:feasibility_program}
%	\begin{array}{>{\displaystyle}c >{\displaystyle}l >{\displaystyle}l}
%		\text{find} & \occ(\grid_1), \ldots, \occ(\grid_G) \in \{0, 1\}^G &\\
%		\text{subject to} & \quad \sum_{\grid_i \in \xi_s^*} \occ(\grid_i) = 0, & \quad \forall s = 1, \ldots, \numsafe \\
%		 & \quad \sum_{\grid_i \in \xi_u} \occ(\grid_i) \ge 1, & \quad \forall u = 1, \ldots, \numunsafe
%	\end{array}
%\end{equation}

Furthermore, one can obtain a conservative estimate of the unsafe set from this feasibility problem by intersecting all solutions to Equation \ref{eq:feasibility_program}. This follows because if the unsafeness of a cell is shared across all feasible solutions, the constraints uniquely define that cell must be occupied:

\begin{proposition}[Integer program conservativeness]
	The intersection of all feasible solutions to Equation \ref{eq:feasibility_program} is a conservative estimate of the unsafe set $\unsafeset$.
\end{proposition}

In practice, it may be difficult to directly find all solutions to the feasibility problem, as in the worst case, finding the set of all feasible solutions is equivalent to exhaustive search in the full gridded space. A more efficient method is to loop over all grid cells and set each one to be safe, and see if the optimizer can still find a feasible solution. Cells where there exists no feasible solution are guaranteed unsafe. This amounts to solving $\vert G \vert$ binary integer feasibility problems, which can be trivially parallelized. Furthermore, any cells that are already known to be safe for sure (from demonstrations) do not need to be checked.

\subsubsection{Incorporating prior knowledge in the integer program}

As will be discussed in detail in Section \ref{sec:learnability}, depending on the cost function, the demonstrations given, and the known constraints, it may not be possible to recover a unique unsafe set. However, we may have some prior on the nature of the unsafe set, such as it being smooth, simply connected, or that the certain regions of the constraint space are unlikely to be unsafe. Assume that this prior knowledge can be encoded in some ``energy" function $E(\cdot, \ldots, \cdot) : \{0, 1 \}^G \rightarrow \reals$ mapping the set of binary occupancies to a scalar value, which indicates the desirability of a particular unsafe set configuration.

By combining these components, we can write a binary integer minimization program to find an unsafe set that is consistent with the occupancies enforced by the safe and unsafe trajectories, and is optimal with respect to the prior (or locally optimal, if $E$ is non-convex):

\begin{equation}\label{eq:integer_program}
	\begin{array}{>{\displaystyle}c >{\displaystyle}l >{\displaystyle}l}
		\underset{\occ(\grid_1), \ldots, \occ(\grid_G) \in \{0, 1\}^G}{\text{minimize}} & \quad E(\occ(\grid_1), \ldots, \occ(\grid_G)) &\\
		\text{subject to} & \quad \sum_{\grid_i \in \xi_s^*} \occ(\grid_i) = 0, & \quad \forall s = 1, \ldots, \numsafe \\
		 & \quad \sum_{\grid_i \in \xi_u} \occ(\grid_i) \ge 1, & \quad \forall u = 1, \ldots, \numunsafe
	\end{array}
\end{equation}


\subsection{Probabilistic setting and continuous relaxation}\label{sec:continuous_relaxation}

The binary occupancy formulation also sets the stage for a probabilistic setting, in which grid cells may be unsafe with some probability of unsafeness, either inherently or due to our uncertainty over its label.

More precisely, consider the case where instead of the occupancy of a cell being an indicator variable, it is instead a random variable $\gridrv_i$, where $\gridrv_i$ takes value $1$ with probability $\occp(\gridrv_i)$ and value $0$ with probability $1-\occp(\gridrv_i)$. Here, the occupancy probability function maps cells to occupancy probabilities $\occp(\cdot) : \gridspace \rightarrow [0, 1]$.

Trajectories in the stochastic case can now be safe or unsafe with some probability. We obtain analogous constraints from the integer program in Section \ref{sec:integer_program} in the probabilistic setting. Known safe trajectories traverse cells that are unsafe with probability 0; this can be enforced with the constraint $\sum_{\gridrv_i \in \xi_s^*} \occp(\gridrv_i) = 0$: if the probabilities of unsafeness are all zero along a trajectory, then the trajectory must be safe. Trajectories that are unsafe with probability $p_u$ satisfy the following constraint:

\begin{equation*}
	\expectation \Bigg[ \sum_{\gridrv_i \in \xi_u} \gridrv_i \Bigg] = \sum_{\gridrv_i \in \xi_u} \occp(\gridrv_i) = (1-p_u)\times 0 + p_u \times S_u \ge p_u
\end{equation*}

\noindent where we denote the sum of occupancies when the trajectory is unsafe as $S_u$, where $S_u \ge 1$.

To avoid a stochastic program optimizing over random variables, we can solve a deterministic optimization problem by optimizing over the occupancy probabilities directly:

\begin{equation}\label{eq:stochastic_program}
	\begin{array}{>{\displaystyle}c >{\displaystyle}l >{\displaystyle}l}
		\underset{\occ(\gridrv_1), \ldots, \occ(\gridrv_G) \in [0, 1]^G}{\text{minimize}} & \quad E(\occ(\gridrv_1), \ldots, \occ(\gridrv_G)) &\\
		\text{subject to} & \quad \sum_{\gridrv_i \in \xi_s^*} \occp(\gridrv_i) = 0, & \quad \forall s = 1, \ldots, \numsafe \\
		 & \quad \sum_{\gridrv_i \in \xi_u} \occp(\gridrv_i) \ge p_u, & \quad \forall u = 1, \ldots, \numunsafe \\
	\end{array}
\end{equation}

This probabilistic formulation also sheds light on the continuous relaxation of the binary integer program in Section \ref{sec:integer_program}. When $p_u = 1$ for all $u$, i.e. the unsafe trajectories are unsafe for sure, the optimization problem in (\ref{eq:stochastic_program}) coincides with the continuous relaxation of the integer program in (\ref{eq:integer_program}). Hence, this provides justification for solving the continuous relaxation and interpreting the output as occupancy probabilities for each cell.

%It is of note that the optimization-based approach simply finds an unsafe set that is consistent with the safe and unsafe trajectories that have been provided or sampled. Because of this, it is possible that the recovered unsafe set is not a conservative estimate of the true unsafe set. However, it is possible to recover a conservative unsafe set by taking the optimization problem and setting a grid cell to be safe and seeing if the optimizer can find a feasible solution; if it cannot, then we refer to that cell as having been ``uniquely learned unsafe". While repeating this procedure for all grid cells can be computationally expensive, this can be trivially parallelizable, and grid cells traversed by the demonstrations and cells that are involved in length $3$ unsafe sub-trajectories (as shown in Section \ref{sec:subtrajectory}) do not need to be checked. However, we note that in our experience, as long as enough safe demonstrations are given and enough unsafe trajectories are sampled, we do not observe much over-approximation.

%Furthermore, assuming the occupancies of cells are independent, a trajectory $\xi_u$ is unsafe with probability $p_u \doteq 1 - \prod_{\grid_i \in \xi_u} (1 - \occ(\grid_i))$. Denote the sum of occupancies when the trajectory is unsafe as $s_u$, where $s_u \ge 1$. Then, the expected sum of occupancies can be written as

%This original constraint is non-convex in $\occ(\grid_i)$ but can be rewritten as a convex constraint via the following procedure:
%
%\begin{equation}
%\begin{aligned}
%	\expectation \Bigg[ \sum_{\grid_i \in \xi_u} \occ(\grid_i) \Bigg] & \ge 1 - \prod_{\grid_i \in \xi_u} (1 - \occ(\grid_i)) \\
%	& \Updownarrow \\
%	\log\Bigg(\expectation \Bigg[ \sum_{\grid_i \in \xi_u} \occ(\grid_i) \Bigg]\Bigg) & \ge \log\Bigg(-\prod_{\grid_i \in \xi_u}(1 - \occ(\grid_i))\Bigg) \\
%	& = \sum_{z_i \in \xi_u} \log(\occ(\grid_i) - 1) \\
%	& \Updownarrow \\
%	0 & \ge \exp\Bigg(\sum_{z_i \in \xi_u} \log(\occ(\grid_i) - 1))\Bigg) - \expectation \Bigg[ \sum_{\grid_i \in \xi_u} \occ(\grid_i) \Bigg]
%\end{aligned}
%\end{equation}
%
%\noindent where the last inequality is convex since it is the difference of a convex function and a linear function.
%
%Furthermore, if we consider the scenario where $p_U$ is given a priori, as in the case of suboptimal demonstrations in Section \ref{sec:suboptimal}, the constraint becomes linear.

\subsection{Bounded suboptimality of demonstrations}

We now consider the case where we are given a $\delta$-suboptimal demonstration $\hat\xi$, where $c(\hat\xi) \le (1+\delta)c(\xi^*)$, where $\xi^*$ is an optimal demonstration.

All the main ideas of the sampling techniques discussed in earlier sections hold, but now we need to be careful that any unsafe trajectories we sample from the intersection are truly infeasible: a sampled trajectory of cost $c\ge c^*$ can be potentially safe. Since we do not know what $c^*$ is, we provide a few methods for still learning conservative estimates of the unsafe set.

Assume first that we have no model on how the demonstrator performs or that we want to guarantee that the recovered unsafe set is guaranteed conservative. In this setting, the only way to obtain any quantifiable guarantees on the conservativeness of the unsafe set is to sample from the sub-level set $\frac{c}{1+\delta}$. This can be highly conservative if $\delta$ is large.

\textcolor{red}{TODO: ADD PROBABILISTIC WRITEUP.}

%However, let's now assume that we have some distribution over how suboptimal a demonstrator behaves: $\prob(c(\xi))$. In reality, this is not too far-fetched, as it's likely that the demonstrator will be provided a few test runs to familiarize him/herself with the setup before performing demonstrations which can be used to estimate $\prob(c(\xi))$. In this case, if we were to sample from the $\frac{c}{1+\delta} + \epsilon$ sub-level set, the 
%
%There is also the setting in which multiple suboptimal demonstrations of the same task are recorded. In this case, if we have a fixed value of $\delta$, we can sample from a higher sub-level set and still 

\subsection{Side information and priors}

\subsubsection{Feature maps}
Oftentimes, we have other sensors that can provide information about the constraint not included in the system state-control trajectory; i.e. we may have \textit{feature data} on the environment or the system. In this case, if the constraint to be learned is also active and well-represented in the features, we can find the unsafe set in the feature space instead. In particular, if the structure of the constraint is much simpler in the feature space than it is directly in the constraint space, learning the constraint in the feature space may both improve sample complexity and learnability. We run an experiment on this in Section \ref{sec:feature_experiment}, where learning the constraint in feature space is trivial compared to a fairly complex constraint in the state space.

\subsubsection{Convex unsafe sets}
If we know that the unsafe set is convex, then the convex hull of the uniquely learned unsafe states is also unsafe. This is because the convex hull of the learned unsafe states is guaranteed to be a subset of the true unsafe set, since the convex hull is the smallest convex set that contains all of the learned unsafe states, and thus is contained within the true unsafe set.

\subsubsection{Negative information}
In case it is also easy for the user to provide information about where in the state space it is impossible to obtain a feasible connecting path, one can sample from the infinite sub-level set intersection.
%\subsubsection{Convex unsafe sets}
%
%\begin{itemize}
%	\item Feature maps
%	\item Convex obstacles
%	\item Gridding ($\approx$ local consistency)
%\end{itemize}
